On the Relationship between Data Efficiency and Error for Uncertainty Sampling

While active learning offers potential cost savings, the actual data efficiency---the reduction in amount of labeled data needed to obtain the same error rate---observed in practice is mixed. This paper poses a basic question: when is active learning actually helpful? We provide an answer for logistic regression with the popular active learning algorithm, uncertainty sampling. Empirically, on 21 datasets from OpenML, we find a strong inverse correlation between data efficiency and the error rate of the final classifier. Theoretically, we show that for a variant of uncertainty sampling, the asymptotic data efficiency is within a constant factor of the inverse error rate of the limiting classifier.

==> zzzz_proof_US_H.tex <==
\begin{@twocolumnfalse}

For any $\epsilon$, define $A(i,\epsilon)$ to be the event that $\|\hat{w}_i - w^*\|_2$

%%%%%%%%%%%%% LEMMA
\begin{lemma}
$$\sum_{i=n_{seed}}^n \Pr[A(i,\epsilon)] \leq L_\epsilon \log(n)$$
\end{lemma}
\begin{proof}

For any $\epsilon$, there exists some $L_\epsilon$
$$\Pr[\|\hat{w}_n - w^*\|_2 \geq \epsilon] \leq \frac{L_{\epsilon}}{n}$$

Therefore,

$$\sum_{i=n_{seed}+1}^n \Pr[A(i,\epsilon)] \leq $$
$$\sum_{i=n_{seed}+1}^n \Pr[\|\hat{w}_i - w^*\|_2 \geq \epsilon] $$
$$\leq L_\epsilon \cdot (1) + \sum_{i= \max(n_{seed}+1,L_\epsilon)}^n \frac{L_\epsilon}{i}$$
$$\leq L_\epsilon + L_\epsilon \log(n) - L_\epsilon \log(L_\epsilon)$$
$$\leq L_\epsilon \log(n)$$

\end{proof}
%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
%Recall that the $10^{th}$ moment of $x$ is bounded, \mus{MAKE THIS ASSUMPTION}

%Let $X_{max}$ be the unlabeled point with the largest magnitude,

%\begin{lemma}
%$$\Pr[\|X_{max}\|^2 > n^{4/5}] = O(n^{-2}) = \delta_1$$
%\end{lemma}
%\begin{proof}
%$$\mathbb{E}[\|x\|^{10}] \leq B$$
%$$R^5 \Pr[ \|x\|^2 > R] \leq B$$

%by union bound,

%$$\Pr[\|X_{max}\|^2 > R] \leq N \Pr[ \|x\|^2 > R]$$
%$$\leq \frac{N B}{R^5}$$

%setting $R=n^{4/5}$, and noting that $N = O(n^2)$, we find,

%$$\Pr[\|X_{max}\|^2 > n^{4/5}] = O(n^{-2}) = \delta_1$$
%\end{proof}
%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%

Define $Q = \sigma (1-\sigma) = \sigma(w^* \cdot x) (1 - \sigma(w^* \cdot x))$.

$$\| \sum_{i=n_{seed}+1}^n \mathbb{E}_{x \sim \hat{w}_i}[Qxx^T] - (n - n_{seed}) \mathbb{E}_{x \sim w^*}[Q xx^T] \|$$
$$= \|\sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | A(i,\epsilon)] \Pr[A(i,\epsilon)] + \sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | \neg A(i,\epsilon)] (1- \Pr[A(i,\epsilon)]) - (n - n_{seed}) \mathbb{E}_{x \sim w^*}[Q xx^T]\|$$

$$\leq \|\sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | A(i,\epsilon)] \Pr[A(i,\epsilon)]\| + \|\sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | \neg A(i,\epsilon)] \Pr[A(i,\epsilon)] \| + $$
$$
+ \| \sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | \neg A(i,\epsilon)] - (n-n_{seed}) \mathbb{E}_{x \sim w^*}[Q xx^T] \|$$
$$\leq 2 (\frac{1}{4} B^2) \sum_i \Pr[A(i,\epsilon)]    +   \| \sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | \neg A(i,\epsilon)] - (n-n_{seed}) \mathbb{E}_{x \sim w^*}[Q xx^T] \|$$
$$\leq \frac{1}{2} B^2 L_\epsilon \log(n) + \| \sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | \neg A(i,\epsilon)] - (n-n_{seed}) \mathbb{E}_{x \sim w^*}[Q xx^T] \|$$

$$\leq \frac{1}{2} B^2 L_\epsilon \log(n) + \| \sum_i \mathbb{E}_{x \sim \hat{w}_i}[Q xx^T | \neg A(i,\epsilon)] - (n-n_{seed}) \mathbb{E}_{x \sim w^*}[Q xx^T]$$


%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
For sufficiently small $\epsilon$, if $\|w' - w^*\|_2 \leq \epsilon$, then

$$|\int_{w'\cdot x = 0} p(x) - \int_{w^* \cdot x = 0} p(x)\| = O(\epsilon)$$
\end{lemma}
\begin{proof}
Without loss of generality (rotation and translation), let $w^*_0=0$, $w^*=\|w^*\|e_1$ and let $w' = w'_1 e_1 + w'_2 e_2$.

We sample from places where $w'_0 + w'_1 x_1 + w'_2 x_2 = 0$ which occurs when $x_1 = \frac{w'_2}{w'_1} x_2 + \frac{w'_0}{w'_1} = ax_2 + b$. From the theorem assumption, we know that $|w'_0|, |w'_2| \leq \epsilon$ and $|w'_1| \geq \|w^*\| - \epsilon \geq 2 \|w^*\|$ (for sufficiently small $\epsilon$) so we know that $|a|, |b| \leq \frac{\epsilon}{2\|w^*\|}$

Note that

$$|\int_{w'\cdot x = 0} p(x) - \int_{w^* \cdot x = 0} p(x)\|=$$

(Note that the Jacobian of the change of variables has the following matrix which has determinant $1$)

$$\begin{bmatrix}
    1 & 0 \\
    -a & 1\\
  \end{bmatrix}
$$


$$=|\int_{x} p(x_1=ax + b,x_2=x) - p(x_1=0)|$$
$$\leq \int_{x} |p(x_1=ax + b|x_2=x)p(x_2=x) - p(x_1=0|x_2=x)p(x_2=x)|$$

With the assumption that the conditional probabilities are Lipschitz,

$$ \leq \int_{x} L |ax + b| p(x_2=x)$$
$$ \leq a L \mathbb{E}[|x_2|] + b L$$
$$ \leq \frac{\epsilon}{2\|w^*\|} L \mathbb{E}[|x_2|] + \frac{\epsilon}{2\|w^*\|} L$$
$$ \leq O(\epsilon)$$
\end{proof}

For small enough $\epsilon$, then $\int_{w'\cdot x = 0} p(x) > p_0/2$ if $\|w' - w^*\|_2 \leq 2\epsilon$. Thus, the probability of there being an unlabeled point within a parallel plane with bias less than $\epsilon$ different from a $\hat{w}$ such that $\|\hat{w} - w^*\|_2 \leq \epsilon$ is at least $2 \frac{\epsilon}{|\hat{w}|} (p_0/2) \geq \frac{\epsilon p_0}{|w^*| - \epsilon}$. The probability of no unlabeled point within this small slice around the plane defined by $\hat{W}$ is

$$(1- \frac{\epsilon p_0}{|w^*| - \epsilon})^(N/n)$$

so the probability of not being able to select such a point (by union bound) is,

$$n(1- \frac{\epsilon p_0}{|w^*| - \epsilon})^(N/n) \leq n \exp(\frac{\epsilon p_0}{|w^*| - \epsilon} \frac{N}{n}) = \delta_2$$

Thus, with high probability, the plane that we sample the point from on the $i^{th}$ iteration given that $i=good$ is within $2 \epsilon$ from $w^*$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
If $\|w' - w^*\|_2 \leq 2 \epsilon$ and $\|w^*\| \geq 3 \epsilon$, then

$$\| \mathbb{E}[\mathbbm{1}[\sigma (1-\sigma) xx^T] - \mathbb{E}_{w^* \cdot x = 0}[\sigma (1-\sigma) xx^T] \| \leq O(\epsilon^2)$$
\end{lemma}
\begin{proof}
Without loss of generality (rotation and translation), let $w^*_0=0$, $w^*=\|w^*\|e_1$ and let $\hat{w} = c_1 e_1 + c_2 e_2$.

We sample from places where $w'_0 + w'_1 x_1 + w'_2 x_2 = 0$ which occurs when $x_1 = \frac{w'_2}{w'_1} x_2 + \frac{w'_0}{w'_1} = ax_2 + b$. From the theorem assumption, we know that $|w'_0|, |w'_2| \leq \epsilon$ and $|w'_1| \geq \|w^*\| - \epsilon \geq 2 \|w^*\|$ so we know that $|a|, |b| \leq \frac{\epsilon}{2\|w^*\|}$

Define $Q(x_1) = \sigma(w^*_1 x_1) \sigma(-w^*_1 x_1)$

For $i_1 + i_2 + ... + i_d \leq 2$,

First, we compute the joint (not the conditionals) and then we can divide by the marginals from the previous lemma,

$$\mathbb{E}_{w' \cdot x = 0}[\sigma (1-\sigma) xx^T]_{i,j} = $$

$$=\mathbb{E}_{w' \cdot x = 0}[Q(x_1) (x_1)^{i_1} (x_2)^{i_2} (x_3)^{i_3} ... ] = $$

(As before, the Jacobian of the change of variables has determinant $1$)
$$\int_{x} p(x_1 = ax + b, x_2=x) Q(ax + b) (ax + b)^{i_1} (x)^{i_2} \mathbb{E}[x_3^{i_3}  ... | x_1 = ax + b, x_2=x]=$$ 
$$ = \int_{x} p(x_2=x) (x)^{i_2} F(ax+b, x)$$

where $F(x_1, x_2) = p(x_1 | x_2)  (Q(x_1) x_1^{i_1}) mathbb{E}[x_3^{i_3}  ... | x_1, x_2]$

\mus{Include these as assumptions}
since all three components of $F$ are bounded and Lipschitz, $F$ is Lipschitz.

$$|\int_{x} p(x_2=x) (x)^{i_2} F(ax+b,x) - \int_{x} p(x_2=x) (x)^{i_2} F(0,x) $$
$$\leq  \int_{x} p(x_2=x) |x|^{i_2} L |ax+b|$$
$$ \leq  a L \mathbb{E}[|x_2|^{i_2+1}|] + b L \mathbb{E}[|x_2|^{i_2}|]$$
$$\leq \frac{\epsilon}{2\|w^*\|} L (B_3 + B_2) = O(\epsilon)$$
\mus{assume third moments in plane are bounded}

Thus, for any $i,j$, 

$$\| \mathbb{E}_{w' \cdot x = 0}[\sigma (1-\sigma) xx^T]_{i,j} - \mathbb{E}_{w^* \cdot x = 0}[\sigma (1-\sigma) xx^T]_{i,j} \| \leq O(\epsilon)$$
$$\|\mathbb{E}_{w' \cdot x = 0}[\sigma (1-\sigma) xx^T]- \mathbb{E}_{w^* \cdot x = 0}[\sigma (1-\sigma) xx^T]\|_F \leq d^2 O(\epsilon^2)$$
$$\|\mathbb{E}_{w' \cdot x = 0}[\sigma (1-\sigma) xx^T]- \mathbb{E}_{w^* \cdot x = 0}[\sigma (1-\sigma) xx^T]\|_2 \leq O(\epsilon^2)$$
\end{proof}

Note that 

$$\|\frac{A}{a} - \frac{B}{b}\| = \|\frac{bA - aB}{ab}\|$$
$$ = \|\frac{a(A-B) - (a-b)A}{ab}\|$$
$$\leq \frac{1}{b} \|A-B\| + \frac{|a-b|}{ab} \|A\|$$
$$ = \frac{1}{b} O(\epsilon^2) + O(\epsilon) \frac{1}{ab}\|A\|$$
$$ = O(\epsilon)$$


\end{@twocolumnfalse}

==> zzzz_remove_first_for_Gaussian.tex <==
\begin{@twocolumnfalse}

Let us use the $-i$ index to refer to all indices except the $i^{th}$ index. For matrices, let $A_{-1}$ be the matrix by deleting the first row and column.

%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
If $x \sim N(\mu, \Sigma)$,
then $x_{-1} | x_1$ is normally distributed with mean

$$\mu_{-1} + \Sigma_{1,-1} \Sigma_{1,1}^{-1} (x_1 - \mu_1),$$

and covariance

$$\Sigma_{-1} - \Sigma_{1,1}^{-1} \Sigma_{1,-1} \Sigma_{1,-1}^T$$

\end{lemma}
\begin{proof}

Let 

$$z = x_{-1} - \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1$$

Note that,

$$Cov(z,x_1) = Cov(x_{-1},x_1) - \Sigma_{1,-1} \Sigma_{1,1}^{-1} Cov(x_1, x_1)$$
$$ = \Sigma_{1,-1} - \Sigma_{1,-1} \Sigma_{1,1}^{-1} \Sigma_{1,1}$$
$$ = 0$$

Since $z$ and $x_1$ are both normally distributed and uncorrelated, they are independent.

$$\mathbb{E}[x_{-1} | x_1] = \mathbb{E}[z + \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1 | x_1]$$
$$=\mathbb{E}[z] + \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1$$
$$=\mathbb{E}[x_{-1}] + \Sigma_{1,-1} \Sigma_{1,1}^{-1} (x_1 - \mathbb{E}[x_1])$$
$$= \mu_{-1} + \Sigma_{1,-1} \Sigma_{1,1}^{-1} (x_1 - \mu_1)$$

Further, 

$$Cov(x_{-1},x_{-1} | x_1) = Cov( z + \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1, z + \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1 | x_1)$$

conditioned on $x_1$, $x_1$ is a constant

$$= Cov(z,z|x_1)$$

since $z$ is independent of $x_1$,

$$= Cov(z,z)$$
$$ = Cov(x_{-1} - \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1,x_{-1} - \Sigma_{1,-1} \Sigma_{1,1}^{-1} x_1)$$
$$ = Cov(x_{-1},x_{-1}) -  2 \Sigma_{1,1}^{-1} \Sigma_{1,-1} \Sigma_{1,-1}^T + \Sigma_{1,1}^{-1}\Sigma_{1,-1} \Sigma_{1,-1}^T $$
$$ = \Sigma_{-1} - \Sigma_{1,1}^{-1} \Sigma_{1,-1} \Sigma_{1,-1}^T$$
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
Denote $Err(\mu, \Sigma)$ as the error by a Gaussian perturbation (around $w^*$) by $N(\mu, \Sigma)$. If $\mu$ is left off, it is zero.

Let $r$ be the strong convexity radius around $w^*$ with strong convexity parameter $m$,

\begin{lemma}
If $\Sigma_1 \succ \Sigma_2$, then

$$Err(\mu,\Sigma_1) \geq \Pr[\|N(0,\Sigma_1-\Sigma_2)\|<\frac{r}{2}] (Err(\mu,\Sigma_2) - \Pr[\|N(\mu,\Sigma_2)\|>\frac{r}{2}])$$

\end{lemma}
\begin{proof}
Denote $\Sigma' = \Sigma_1 - \Sigma_2 \succ 0$

$$Err(\mu,\Sigma_1) = Err(\mu,\Sigma_2 + \Sigma')$$
$$ = \int_{w} p_{\mu,\Sigma_2 + \Sigma'}(w) Err(w)$$
$$ = \int_{w} \int_{w'} p_{\mu,\Sigma_2}(w) p_{0,\Sigma'}(w') Err(w + w')$$
$$ \geq \int_{\|w\| < \frac{r}{2}} \int_{\|w'\| < \frac{r}{2}} p_{\mu,\Sigma_2}(w) p_{0,\Sigma'}(w') \frac{1}{2}(Err(w + w') + Err(w - w'))$$
$$ \geq \int_{\|w\| < \frac{r}{2}} \int_{\|w'\| < \frac{r}{2}} p_{\mu,\Sigma_2}(w) p_{0,\Sigma'}(w') (Err(w) + \frac{1}{2} m \|w'\|^2)$$

This is composed of two pieces, the first piece,

$$\int_{\|w\| < \frac{r}{2}} \int_{\|w'\| < \frac{r}{2}} p_{\mu,\Sigma_2}(w) p_{0,\Sigma'}(w') Err(w) = $$
$$= \Pr[\|N(0,\Sigma')\|<\frac{r}{2}] \int_{\|w\| < \frac{r}{2}} p_{\mu,\Sigma_2}(w) Err(w)$$
$$= \Pr[\|N(0,\Sigma')\|<\frac{r}{2}] (Err(\mu,\Sigma_2) - \int_{\|w\| > \frac{r}{2}} p_{\mu,\Sigma_2}(w) Err(w))$$
$$\geq \Pr[\|N(0,\Sigma')\|<\frac{r}{2}] (Err(\mu,\Sigma_2) - \Pr[\|N(\mu,\Sigma_2)\|>\frac{r}{2}])$$

The second piece is,

$$\int_{\|w\| < \frac{r}{2}} \int_{\|w'\| < \frac{r}{2}} p_{\mu,\Sigma_2}(w) p_{0,\Sigma'}(w') \frac{1}{2} m \|w'\|^2$$
$$= \frac{1}{2} m \Pr[\|N(\mu,\Sigma_2)\|<\frac{r}{2}] \int_{\|w'\| < \frac{r}{2}} p_{0,\Sigma'}(w') \|w'\|^2$$



\end{proof}
%%%%%%%%%%%%%%%%%
\begin{lemma}
For $\alpha>1$, if $\alpha \mu < r/2$

$$Err(\alpha \mu,\alpha^2 \Sigma) \geq Err(\mu,\Sigma) - \Pr[\|N(\alpha \mu, \alpha^2 \Sigma)\| > r]$$
\end{lemma}
\begin{proof}

$$Err(\alpha \mu,\alpha^2 \Sigma) = \int_{w} p_{\alpha \mu,\alpha^2 \Sigma}(w) Err(w)$$
$$ = \int_{w} p_{\mu,\Sigma}(w) Err(\alpha w)$$
$$ \geq \int_{\alpha \|w\| < r} p_{\mu,\Sigma}(w)  Err(\alpha w)$$
$$ = \int_{\alpha \|w\| < r} p_{\mu,\Sigma}(w) (\frac{1}{\alpha} Err(\alpha w) + \frac{\alpha - 1}{\alpha} Err(\alpha w))$$
$$ = \int_{\alpha \|w\| < r} p_{\mu,\Sigma}(w) (\frac{1}{\alpha} Err(\alpha w) + \frac{\alpha - 1}{\alpha} Err(\alpha w))$$
$$ \geq \int_{\alpha \|w\| < r} p_{\mu,\Sigma}(w) (\frac{1}{\alpha} Err(\alpha w) + \frac{\alpha - 1}{\alpha} Err(0))$$
$$ \geq \int_{\alpha \|w\| < r} p_{\mu,\Sigma}(w) Err(w)$$
$$ = Err(\mu,\Sigma) - \int_{\alpha \|w\| > r} p_{\mu,\Sigma}(w) Err(w)$$
$$ \geq Err(\mu,\Sigma) - \Pr[\|N(\alpha \mu, \alpha^2 \Sigma)\| > r]$$
\end{proof}

%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%

\begin{lem}[\ref{lem:remove_first}]
$\forall \epsilon$,

$$Err(\Sigma) \geq Err(\frac{1}{(1 + \epsilon )^2} \Sigma_{-1}) - R(\epsilon, \Sigma)$$


$$Err(\Sigma) \leq R(\epsilon, \Sigma) + Err(\frac{1}{(1 - \epsilon)^2}) \Sigma_{-1})$$

where 

$$R(\epsilon, \Sigma) = 2\Phi( -\frac{\epsilon \|w^*\|}{\sqrt{\Sigma_{1,1}}}) + \Pr[\|N(\frac{\epsilon \|w^*\| }{1 - \epsilon} \Sigma_{1,1}^{-1} \Sigma_{1,-1}, \frac{1}{(1 - \epsilon)^2} (\Sigma_{-1} - \Sigma_{1,1}^{-1} \Sigma_{1,-1} \Sigma_{1,-1}^T))\| > r]$$
\end{lem}

\begin{proof}

$$Err(\Sigma) = \mathbb{E}_{w \sim N(w^*,\Sigma)}[Err(w)]$$
$$ = \Pr_{x,y,\Delta w \sim N(0,\Sigma)}[y (w^* + \Delta w) x < 0]$$
$$ = \Pr_{x,y,\Delta w \sim N(0,\Sigma)}[y (w^*_1 + \Delta w_1) x_1 + y \Delta w_{-1} x_{-1} < 0]$$
$$ = \Pr_{x,y,\Delta w \sim N(0,\Sigma)}[y \|w^*\|  x_1 + y \frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} \Delta w_{-1} x_{-1} < 0]$$
$$ = \Pr_{x,y,\Delta w \sim N(0,\Sigma)}[y \|w^*\|  x_1 + y \frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} \Delta w_{-1} x_{-1} < 0]$$

Let $s = \Sigma_{1,1}^{-1} \Sigma_{1,-1}$ and $\Sigma'=\Sigma_{-1} - \Sigma_{1,1}^{-1} \Sigma_{1,-1} \Sigma_{1,-1}^T$. Then,

$$ = \int_{\Delta w_1} p_{N(0,\Sigma_{1,1})}(\Delta w_1) \Pr_{x,y,\Delta w_{-1} \sim N( s \Delta w_1, \Sigma')}[y \|w^*\|  x_1 + y \frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} \Delta w_{-1} x_{-1} < 0]$$
$$ = \int_{\Delta w_1} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)})^2 \Sigma')$$

We can bound this in two directions:

$$Err(\Sigma)  = \int_{\Delta w_1} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)})^2 \Sigma')$$
$$ \leq \Pr[|N(0,\Sigma_{1,1})| > \epsilon \|w^*\|] + \int_{|\Delta w_1| <\epsilon \|w^*\|} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)})^2 \Sigma')$$
$$ \leq 2\Phi( -\frac{\epsilon \|w^*\|}{\sqrt{\Sigma_{1,1}}})  +  \int_{|\Delta w_1| <\epsilon \|w^*\|} p_{N(0,\Sigma_{1,1})}(\Delta w_1) [Err(\frac{\|w^*\|}{\|w^*\| - \epsilon \|w^*\|} s \Delta w_1, (\frac{\|w^*\|}{\|w^*\| - \epsilon \|w^*\|})^2 \Sigma') + $$ $$\Pr[\|N(\frac{\|w^*\|}{\|w^*\| - \epsilon \|w^*\|} s \Delta w_1, (\frac{\|w^*\|}{\|w^*\| - \epsilon \|w^*\|})^2 \Sigma')\| > r]]$$
$$ \leq 2\Phi( -\frac{\epsilon \|w^*\|}{\sqrt{\Sigma_{1,1}}}) + \Pr[\|N(\frac{\epsilon \|w^*\| }{1 - \epsilon} s, \frac{1}{(1 - \epsilon)} \Sigma')\| > r] +  \int_{\Delta w_1} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{1}{1 - \epsilon} s \Delta w_1, \frac{1}{(1 - \epsilon)^2} \Sigma')$$

Undoing the conditioning on $x_1$,

$$ = R(\epsilon, \Sigma) + Err(\frac{1}{(1 - \epsilon)^2}) \Sigma_{-1})$$

%%%%%%%%


In the other direction,

$$Err(\Sigma)  = \int_{\Delta w_1} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)})^2 \Sigma')$$
$$ \geq \int_{|\Delta w_1| < \epsilon \|w^*\|} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \Delta w_1)})^2 \Sigma')$$

$$ \geq \int_{|\Delta w_1| < \epsilon \|w^*\|} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \epsilon\|w^*\|)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \epsilon\|w^*\|)})^2 \Sigma') - $$ $$\Pr[\|N(\frac{\|w^*\|}{\|w^*\| + \Delta w_1} s \Delta w_1, (\frac{\|w^*\|}{\|w^*\| + \Delta w_1})^2 \Sigma')\| > r]]$$

$$ \geq \int_{\Delta w_1} p_{N(0,\Sigma_{1,1})}(\Delta w_1) Err(\frac{\|w^*\|}{(\|w^*\| + \epsilon \|w^*\|)} s \Delta w_1, (\frac{\|w^*\|}{(\|w^*\| + \epsilon \|w^*\|)})^2 \Sigma') - \Pr[|N(0,\Sigma_{1,1})| > \epsilon\|w^*\|] - $$ $$ \Pr[\|N(\frac{\|w^*\|}{\|w^*\| - \epsilon \|w^*\|} s \epsilon \|w^*\|, (\frac{\|w^*\|}{\|w^*\| - \epsilon\|w^*\|})^2 \Sigma')\| > r]$$

Undoing the conditioning on $x_1$,

$$ = Err(\frac{1}{(1 + \epsilon )^2} \Sigma_{-1}) - R(\epsilon, \Sigma)$$


\end{proof}


\pagebreak























\end{@twocolumnfalse}
